Flow-Based Synthesis of Reactive Tests for Discrete Decision-Making Systems with Temporal Logic Specifications

Designing tests to evaluate if a given autonomous system satisfies complex specifications is challenging due to the complexity of these systems. This work proposes a flow-based approach for reactive test synthesis from temporal logic specifications, enabling the synthesis of test environments consisting of static and reactive obstacles and dynamic test agents. The temporal logic specifications describe desired test behavior, including system requirements as well as a test objective that is not revealed to the system. The synthesized test strategy places restrictions on system actions in reaction to the system state. The tests are minimally restrictive and accomplish the test objective while ensuring realizability of the system's objective without aiding it (semi-cooperative setting). Automata theory and flow networks are leveraged to formulate a mixed-integer linear program (MILP) to synthesize the test strategy. For a dynamic test agent, the agent strategy is synthesized for a GR(1) specification constructed from the solution of the MILP. If the specification is unrealizable by the dynamics of the test agent, a counterexample-guided approach is used to resolve the MILP until a strategy is found. This flow-based, reactive test synthesis is conducted offline and is agnostic to the system controller. Finally, the resulting test strategy is demonstrated in simulation and experimentally on a pair of quadrupedal robots for a variety of specifications.

==> bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TAC/figures/author_figs/jg_small.jpg}}]{Josefine B. Graebener} (Student Member, IEEE) received a B.Eng. in Aerospace Engineering in 2017 from the Aachen University of Applied Sciences (FH Aachen) in Aachen, Germany, and a M.S. in Space Engineering from California Institute of Technology in 2019. Currently, she is a Ph.D. candidate in Space Engineering with a minor in Computer Science at the California Institute of Technology. Her research interest lies in using formal methods for test and evaluation of autonomous systems, and system diagnostics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TAC/figures/author_figs/apurva_pic.jpg}}]{Apurva Badithela}(Student Member, IEEE) received a Bachelors degree in Aerospace Engineering and Mechanics in 2018 from the University of Minnesota, Twin-Cities. Currently, she is a Ph.D. candidate in Control and Dynamical Systems at the California Institute of Technology. Her dissertation work focuses on Formal Test Synthesis and System-level Evaluation for Safety-Critical Autonomous Systems.  
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TAC/figures/author_figs/deni_small.jpg}}]{Denizalp Goktas} (Member, IEEE), photograph and biography not available at the
time of publication.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TAC/figures/author_figs/wyatt_pic.pdf}}]
{Wyatt Ubellacker} (Member, IEEE), photograph and biography not available at the
time of publication.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TAC/figures/author_figs/eric_small.png}}]
{Eric V. Mazumdar} (Member, IEEE) received a B.S. degree in Computer Science from the Massachusetts Institute of Technology (MIT) in 2015, and a Ph.D in Electrical Engineering and Computer Science from UC Berkeley in 2021.

Currently he is an Assistant Professor in Computing and Mathematical Sciences and Economics at Caltech. His research interests lie at the intersection of machine learning and economics, focusing on developing theoretical foundations and tools to confidently deploy machine learning algorithms into societal systems, particularly in settings with uncertain, dynamic environments in which learning algorithms interact with strategic agents.

Dr. Mazumdar received the NSF CAREER Award in 2023 as well as a Research Fellowship for Learning in Games from the Simons Institute for Theoretical Computer Science.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TAC/figures/author_figs/aaron_pic.pdf}}]
{Aaron D. Ames} (Fellow, IEEE) received a B.S. degree in Mechanical Engineering and a B.A. degree in Mathematics from the University of St. Thomas in 2001, and a M.A. degree in Mathematics and a Ph.D. in Electrical Engineering and Computer Sciences from UC Berkeley in 2006.

Currently he is the Bren Professor of Mechanical and Civil Engineering and Control and Dynamical Systems at the California Institute of Technology. Prior to joining Caltech, he was an Associate Professor in Mechanical Engineering and Electrical \& Computer Engineering at the Georgia Institute of Technology. He was as a Postdoctoral Scholar in Control and Dynamical Systems at Caltech from 2006 to 2008, and began is faculty career at Texas A\&M University in 2008. His research interests span the areas of robotics, nonlinear control and hybrid systems, with a special focus on applications to bipedal robotic walking—both formally and through experimental validation.

Dr. Ames was the recipient of the 2005 Leon O. Chua Award for achievement in nonlinear science at UC Berkeley, and the 2006 Bernard Friedman Memorial Prize in Applied Mathematics. Dr. Ames received the NSF CAREER award in 2010, and the Donald P. Eckman Award in 2015, and the 2019 Antonio Ruberti Young Researcher Prize.\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TAC/figures/author_figs/richard_pic.pdf}}]
{Richard M. Murray} (Fellow, IEEE) received the B.S. degree in Electrical Engineering from California Institute of Technology in 1985 and the M.S. and Ph.D. degrees in Electrical Engineering and Computer Sciences from the University of California, Berkeley, in 1988 and 1991, respectively.

He is currently the Thomas E. and Doris Everhart Professor of Control \& Dynamical Systems and Bioengineering at Caltech. Murray's research is in the application of feedback and control to networked systems, with applications in synthetic biology and autonomy. Current projects include design and implementation of synthetic cells and design, verification, and test synthesis for discrete decision-making protocols for safety-critical, reactive control systems.

Dr. Murray's professional awards include the Richard P. Feynman-Hughes Faculty Fellowship in 1993, awarded annually to an outstanding young faculty member in Engineering and Applied Science at Caltech, the National Science Foundation Early Faculty Career Development (CAREER) Award in 1995, the Office of Naval Research Young Investigator Award in 1995 and the Donald P. Eckman Award in 1997. He is a Fellow of the Institute for Electrical and Electronics Engineers (IEEE) and holds an honorary doctorate from Lund University in Sweden. He is an elected member of the National Academy of Engineering (2013). Dr. Murray received the IEEE Bode Lecture Prize in 2016, the IEEE Control Systems Award in 2017, and the AACC John R. Ragazzini Education Award in 2019.

\end{IEEEbiography}

%% OrCID IDs:
% Apurva: https://orcid.org/0000-0002-9788-2702
% Wyatt: https://orcid.org/0000-0002-4732-6185

==> tab_random_runtimes.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{1.5pt}
\caption{Random Runtime Experiments (Reactive)}
\label{tab:rand_rt_reactive}
\begin{tabular}{|lc|*{4}{cc|}}
\hline
\multicolumn{2}{|c|}{Experiment} & \multicolumn{2}{c|}{$5 \times 5$, $\vert T_{\sys} \vert = (25,100)$} & \multicolumn{2}{c|}{$10 \times 10$, $\vert T_{\sys} \vert = (100,455)$} & \multicolumn{2}{c|}{$15 \times 15$, $\vert T_{\sys} \vert = (225,1060)$} & \multicolumn{2}{c|}{$20 \times 20$, $\vert T_{\sys} \vert = (400,1915)$} \\
\hline
% \cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}\cmidrule(lr){16-18}\cmidrule(lr){19-21}
\multicolumn{1}{|c}{$\vert AP \vert$} & {$\vert \mc{B}_{\pi} \vert$}  & {Graph[s]} & {Opt[s]} & {Graph[s]} & {Opt[s]}  & {Graph[s]} & {Opt[s]}  & {Graph[s]} & {Opt[s]} \\
\hline
\hline
\multicolumn{10}{|l|}{\textbf{Reachability}: $\varphi_\sys = \Feventually p_0$ and $\varphi_\test = \bigwedge_{i=1}^n \Feventually p_i$, $\vert AP \vert = \vert p_0, \ldots, p_n \vert$}\\
\hline
2 & (4, 9) & 0.046$\,\pm\,$ 0.001 & 5.625$\,\pm\,$13.434  & 0.224$\,\pm\,$ 0.0056 & 64.615$\,\pm\,$38.752 & 0.554$\,\pm\,$ 0.009 & 67.383$\,\pm\,$25.467  & 1.078$\,\pm\,$ 0.011 & 68.634$\,\pm\,$31.118 \\

3 & (8, 27) & 0.344$\,\pm\,$ 0.007 & 23.364$\,\pm\,$38.147 & 1.661$\,\pm\,$ 0.022 & 61.684$\,\pm\,$35.119 & 4.004$\,\pm\,$ 0.048 & 91.537$\,\pm\,$31.410  & 7.376$\,\pm\,$ 0.061 & 117.821$\,\pm\,$34.885  \\
\hline
\hline
\multicolumn{10}{|l|}{\textbf{Reachability \& Reaction}: $\varphi_\sys = \Feventually p_1 \bigwedge_{i=2}^n \square(p_i \rightarrow \Feventually q_i)$ and $\varphi_\test = \Feventually p_0 \bigwedge_{i=2} \Feventually p_i$, $\vert AP \vert = \vert p_0, \ldots, p_n, q_2,\ldots, q_n \vert$}\\
\hline
3 & (6, 21) & 0.090$\,\pm\,$ 0.001 & 5.969$\,\pm\,$13.209 & 0.424$\,\pm\,$ 0.016 & 61.063$\,\pm\,$34.646  & 1.037$\,\pm\,$ 0.004 & 71.635$\,\pm\,$41.028 & 2.044$\,\pm\,$ 0.013 & 85.204$\,\pm\,$19.492 \\
5 & (20, 155)  & 1.628$\,\pm\,$ 0.087 & 17.193$\,\pm\,$25.510  & 7.560$\,\pm\,$ 0.023 & 78.439$\,\pm\,$34.705  & 18.019$\,\pm\,$ 0.129 & 159.914$\,\pm\,$76.631  & 33.539$\,\pm\,$ 0.144 & 280.157$\,\pm\,$148.880  \\
\hline
\hline
\multicolumn{10}{|l|}{\textbf{Reachability \& Safety}: $\varphi_\sys = \Feventually p_1 \bigwedge_{i=2}^n \square \neg p_i $ and $\varphi_\test = \Feventually p_0$, $\vert AP \vert = \vert p_0, \ldots, p_n \vert$}\\
\hline
3 & (6, 18) & 0.102$\,\pm\,$ 0.002 & 0.763$\,\pm\,$1.519  & 0.508$\,\pm\,$ 0.010 & 70.818$\,\pm\,$89.697  & 1.278$\,\pm\,$ 0.022 & 63.676$\,\pm\,$27.536 & 2.557$\,\pm\,$ 0.023 & 80.579$\,\pm\,$20.790 \\ 

4 & (6, 18) & 0.116$\,\pm\,$ 0.002 & 0.150$\,\pm\,$0.294  & 0.590$\,\pm\,$ 0.009 & 71.474$\,\pm\,$80.614  & 1.485$\,\pm\,$ 0.024 & 59.591$\,\pm\,$38.918  & 2.918$\,\pm\,$ 0.046 & 76.015$\,\pm\,$27.107  \\
\hline
\end{tabular}
\end{table*}

==> tab_random_static.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{1.5pt}
\caption{Random Runtime Experiments (Static)}
\label{tab:rand_rt_static}
\begin{tabular}{|lc|*{4}{cc|}}
\hline
\multicolumn{2}{|c|}{Experiment} & \multicolumn{2}{c|}{$5 \times 5$, $\vert T_{\sys} \vert = (25,100)$} & \multicolumn{2}{c|}{$10 \times 10$, $\vert T_{\sys} \vert = (100,455)$} & \multicolumn{2}{c|}{$15 \times 15$, $\vert T_{\sys} \vert = (225,1060)$} & \multicolumn{2}{c|}{$20 \times 20$, $\vert T_{\sys} \vert = (400,1915)$} \\
%& \multicolumn{3}{c|}{$25 \times 25$} & \multicolumn{3}{c|}{$30 \times 30$}\\
\hline
% \cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}\cmidrule(lr){16-18}\cmidrule(lr){19-21}
\multicolumn{1}{|c}{$\vert AP \vert$} & {$\vert \mc{B}_{\pi} \vert$}  & {Graph[s]} & {Opt[s]} & {Graph[s]} & {Opt[s]}  & {Graph[s]} & {Opt[s]}  & {Graph[s]} & {Opt[s]} \\
% & {Graph[s]} & {Opt[s]} & {N} & {Graph[s]} & {Opt[s]} & {N} \\
\hline
\hline
\multicolumn{10}{|l|}{\textbf{Reachability}: $\varphi_\sys = \Feventually p_0$ and $\varphi_\test = \bigwedge_{i=1}^n \Feventually p_i$, $\vert AP \vert = \vert p_0, \ldots, p_n \vert$}\\
\hline
2 & (4, 9) &  0.047$\,\pm\,$ 0.001 & 8.167$\,\pm\,$13.144  & 0.228$\,\pm\,$ 0.016 & 54.066$\,\pm\,$17.980  & 0.560$\,\pm\,$ 0.019 & 60.168$\,\pm\,$0.120  & 1.091$\,\pm\,$ 0.016 & 60.172$\,\pm\,$0.101  \\

3 & (8, 27) & 0.490$\,\pm\,$ 0.012 & 27.783$\,\pm\,$21.705 & 1.854$\,\pm\,$ 0.299 & 60.167 $\,\pm\,$0.097 & 4.000$\,\pm\,$ 0.061 & 60.484$\,\pm\,$0.859 & 7.364$\,\pm\,$ 0.064 & 74.023$\,\pm\,$38.705 \\
\hline
\hline
\multicolumn{10}{|l|}{\textbf{Reachability \& Reaction}: $\varphi_\sys = \Feventually p_1 \bigwedge_{i=2}^n \square(p_i \rightarrow \Feventually q_i)$ and $\varphi_\test = \Feventually p_0 \bigwedge_{i=2} \Feventually p_i$, $\vert AP \vert = \vert p_0, \ldots, p_n, q_2,\ldots, q_n \vert$}\\
\hline
3 & (6, 21) & 0.091$\,\pm\,$ 0.001 & 10.619$\,\pm\,$14.855 & 0.421$\,\pm\,$ 0.006 & 60.087$\,\pm\,$0.061  & 1.039$\,\pm\,$ 0.018 & 60.225$\,\pm\,$0.237  & 2.048$\,\pm\,$ 0.017 & 60.342$\,\pm\,$0.457  \\
5 & (20, 155) & 1.648$\,\pm\,$ 0.021 & 20.412$\,\pm\,$19.212 & 7.639$\,\pm\,$ 0.063 & 67.766$\,\pm\,$31.900 & 18.004$\,\pm\,$ 0.046 & 95.352$\,\pm\,$116.823  & 33.530$\,\pm\,$ 0.132 & 268.682$\,\pm\,$222.412\\
%5 & (10,20)  & \(12.3 \pm 3.0\) & \(12.3 \pm 3.0\) & 34.6 & \(12.3 \pm 3.0\) & \(12.3 \pm 3.0\) & 0 & 0 & 0 & 0 & 0 & 0 & 0.1 \\
\hline
\hline
\multicolumn{10}{|l|}{\textbf{Reachability \& Safety}: $\varphi_\sys = \Feventually p_1 \bigwedge_{i=2}^n \square \neg p_i $ and $\varphi_\test = \Feventually p_0$, $\vert AP \vert = \vert p_0, \ldots, p_n \vert$}\\
\hline
3 & (6, 18) & 0.101$\,\pm\,$ 0.002 & 1.272$\,\pm\,$1.471 & 0.504$\,\pm\,$ 0.004 & 60.078$\,\pm\,$0.060 & 1.279$\,\pm\,$ 0.026 & 57.268$\,\pm\,$12.606  & 2.558$\,\pm\,$ 0.019 & 60.317$\,\pm\,$0.237 \\
4 & (6, 18) & 0.117$\,\pm\,$ 0.002 & 0.172$\,\pm\,$0.231 & 0.588$\,\pm\,$ 0.004 & 60.063$\,\pm\,$0.052 & 1.477$\,\pm\,$ 0.037 & 60.141$\,\pm\,$0.103 & 2.906$\,\pm\,$ 0.022 & 60.296$\,\pm\,$0.188 \\
\hline
\end{tabular}
\end{table*}
